Adinkra Symbol Recognition using Classical Machine Learning and Deep Learning

Artificial intelligence (AI) has emerged as a transformative influence, engendering paradigm shifts in global societies, spanning academia and industry. However, in light of these rapid advances, addressing the underrepresentation of black communities and African countries in AI is crucial. Boosting enthusiasm for AI can be effectively accomplished by showcasing straightforward applications around tasks like identifying and categorizing traditional symbols, such as Adinkra symbols, or familiar objects within the community. In this research endeavor, we dived into classical machine learning and harnessed the power of deep learning models to tackle the intricate task of classifying and recognizing Adinkra symbols. The idea led to a newly constructed ADINKRA dataset comprising 174,338 images meticulously organized into 62 distinct classes, each representing a singular and emblematic symbol. We constructed a CNN model for classification and recognition using six convolutional layers, three fully connected (FC) layers, and optional dropout regularization. The model is a simpler and smaller version of VGG, with fewer layers, smaller channel sizes, and a fixed kernel size. Additionally, we tap into the transfer learning capabilities provided by pre-trained models like VGG and ResNet. These models assist us in both classifying images and extracting features that can be used with classical machine learning models. We assess the model's performance by measuring its accuracy and convergence rate and visualizing the areas that significantly influence its predictions. These evaluations serve as a foundational benchmark for future assessments of the ADINKRA dataset. We hope this application exemplar inspires ideas on the various uses of AI in organizing our traditional and modern lives.

==> references.tex <==
@inproceedings{kour2014real,
  title={Real-time segmentation of on-line handwritten arabic script},
  author={Kour, George and Saabne, Raid},
  booktitle={Frontiers in Handwriting Recognition (ICFHR), 2014 14th International Conference on},
  pages={417--422},
  year={2014},
  organization={IEEE}
}

@inproceedings{kour2014fast,
  title={Fast classification of handwritten on-line Arabic characters},
  author={Kour, George and Saabne, Raid},
  booktitle={Soft Computing and Pattern Recognition (SoCPaR), 2014 6th International Conference of},
  pages={312--318},
  year={2014},
  organization={IEEE}
}

@article{hadash2018estimate,
  title={Estimate and Replace: A Novel Approach to Integrating Deep Neural Networks with Existing Applications},
  author={Hadash, Guy and Kermany, Einat and Carmeli, Boaz and Lavi, Ofer and Kour, George and Jacovi, Alon},
  journal={arXiv preprint arXiv:1804.09028},
  year={2018}
}

@article{stone2022artificial,
  title={Artificial intelligence and life in 2030: the one hundred year study on artificial intelligence},
  author={Stone, Peter and Brooks, Rodney and Brynjolfsson, Erik and Calo, Ryan and Etzioni, Oren and Hager, Greg and Hirschberg, Julia and Kalyanakrishnan, Shivaram and Kamar, Ece and Kraus, Sarit and others},
  journal={arXiv preprint arXiv:2211.06318},
  year={2022}
}

@article{shaheen2021applications,
  title={Applications of Artificial Intelligence (AI) in healthcare: A review},
  author={Shaheen, Mohammed Yousef},
  journal={ScienceOpen Preprints},
  year={2021},
  publisher={ScienceOpen}
}

@article{secinaro2021role,
  title={The role of artificial intelligence in healthcare: a structured literature review},
  author={Secinaro, Silvana and Calandra, Davide and Secinaro, Aurelio and Muthurangu, Vivek and Biancone, Paolo},
  journal={BMC medical informatics and decision making},
  volume={21},
  pages={1--23},
  year={2021},
  publisher={Springer}
}

@article{rajpurkar2022ai,
  title={AI in health and medicine},
  author={Rajpurkar, Pranav and Chen, Emma and Banerjee, Oishi and Topol, Eric J},
  journal={Nature medicine},
  volume={28},
  number={1},
  pages={31--38},
  year={2022},
  publisher={Nature Publishing Group US New York}
}

@article{yan2022machine,
  title={Machine learning Fundamentals},
  author={Yan, Yan},
  journal={Machine Learning in Chemical Safety and Health: Fundamentals with Applications},
  pages={19--46},
  year={2022},
  publisher={Wiley Online Library}
}

@article{fatemidokht2021efficient,
  title={Efficient and secure routing protocol based on artificial intelligence algorithms with UAV-assisted for vehicular ad hoc networks in intelligent transportation systems},
  author={Fatemidokht, Hamideh and Rafsanjani, Marjan Kuchaki and Gupta, Brij B and Hsu, Ching-Hsien},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={22},
  number={7},
  pages={4757--4769},
  year={2021},
  publisher={IEEE}
}

@article{pamucar2022metaverse,
  title={A metaverse assessment model for sustainable transportation using ordinal priority approach and Aczel-Alsina norms},
  author={Pamucar, Dragan and Deveci, Muhammet and Gokasar, Ilgin and Tavana, Madjid and K{\"o}ppen, Mario},
  journal={Technological Forecasting and Social Change},
  volume={182},
  pages={121778},
  year={2022},
  publisher={Elsevier}
}

@article{goodell2021artificial,
  title={Artificial intelligence and machine learning in finance: Identifying foundations, themes, and research clusters from bibliometric analysis},
  author={Goodell, John W and Kumar, Satish and Lim, Weng Marc and Pattnaik, Debidutta},
  journal={Journal of Behavioral and Experimental Finance},
  volume={32},
  pages={100577},
  year={2021},
  publisher={Elsevier}
}

@article{dowling2023chatgpt,
  title={ChatGPT for (finance) research: The Bananarama conjecture},
  author={Dowling, Michael and Lucey, Brian},
  journal={Finance Research Letters},
  volume={53},
  pages={103662},
  year={2023},
  publisher={Elsevier}
}

@article{zhang2021ai,
  title={AI technologies for education: Recent research \& future directions},
  author={Zhang, Ke and Aslan, Ayse Begum},
  journal={Computers and Education: Artificial Intelligence},
  volume={2},
  pages={100025},
  year={2021},
  publisher={Elsevier}
}

@article{holmes2021ethics,
  title={Ethics of AI in education: Towards a community-wide framework},
  author={Holmes, Wayne and Porayska-Pomsta, Kaska and Holstein, Ken and Sutherland, Emma and Baker, Toby and Shum, Simon Buckingham and Santos, Olga C and Rodrigo, Mercedes T and Cukurova, Mutlu and Bittencourt, Ig Ibert and others},
  journal={International Journal of Artificial Intelligence in Education},
  pages={1--23},
  year={2021},
  publisher={Springer}
}

@article{cope2021artificial,
  title={Artificial intelligence for education: Knowledge and its assessment in AI-enabled learning ecologies},
  author={Cope, Bill and Kalantzis, Mary and Searsmith, Duane},
  journal={Educational Philosophy and Theory},
  volume={53},
  number={12},
  pages={1229--1245},
  year={2021},
  publisher={Taylor \& Francis}
}

@INPROCEEDINGS{9443970,
  author={Adjeisah, Michael and Liu, Guohua and Nortey, Richard Nuetey and Song, Jinling and Lamptey, Khalid Odartey and Frimpong, Felix Nana},
  booktitle={2020 IEEE Intl Conf on Parallel & Distributed Processing with Applications, Big Data & Cloud Computing, Sustainable Computing & Communications, Social Computing & Networking (ISPA/BDCloud/SocialCom/SustainCom)}, 
  title={Twi Corpus: A Massively Twi-to-Handful Languages Parallel Bible Corpus}, 
  year={2020},
  volume={},
  number={},
  pages={1043-1049},
  doi={10.1109/ISPA-BDCloud-SocialCom-SustainCom51426.2020.00157}}

@article{adjeisah2021pseudotext,
  title={Pseudotext injection and advance filtering of low-resource corpus for neural machine translation},
  author={Adjeisah, Michael and Liu, Guohua and Nyabuga, Douglas Omwenga and Nortey, Richard Nuetey and Song, Jinling and others},
  journal={Computational Intelligence and Neuroscience},
  volume={2021},
  year={2021},
  publisher={Hindawi}
}

@article{rivera2022machine,
  title={Machine translation systems and quality assessment: a systematic review},
  author={Rivera-Trigueros, Irene},
  journal={Language Resources and Evaluation},
  volume={56},
  number={2},
  pages={593--619},
  year={2022},
  publisher={Springer}
}


@article{bayoudh2021transfer,
  title={Transfer learning based hybrid 2D-3D CNN for traffic sign recognition and semantic road detection applied in advanced driver assistance systems},
  author={Bayoudh, Khaled and Hamdaoui, Fay{\c{c}}al and Mtibaa, Abdellatif},
  journal={Applied Intelligence},
  volume={51},
  pages={124--142},
  year={2021},
  publisher={Springer}
}

@article{haque2021deepthin,
  title={DeepThin: A novel lightweight CNN architecture for traffic sign recognition without GPU requirements},
  author={Haque, Wasif Arman and Arefin, Samin and Shihavuddin, ASM and Hasan, Muhammad Abul},
  journal={Expert Systems with Applications},
  volume={168},
  pages={114481},
  year={2021},
  publisher={Elsevier}
}

@article{murthy2022efficientlitedet,
  title={EfficientLiteDet: a real-time pedestrian and vehicle detection algorithm},
  author={Murthy, Chintakindi Balaram and Hashmi, Mohammad Farukh and Keskar, Avinash G},
  journal={Machine Vision and Applications},
  volume={33},
  number={3},
  pages={47},
  year={2022},
  publisher={Springer}
}

@incollection{islam2022machine,
  title={Machine learning in computer vision},
  author={Islam, ABM Rezbaul},
  booktitle={Applications of Machine Learning and Artificial Intelligence in Education},
  pages={48--72},
  year={2022},
  publisher={IGI Global}
}

@article{guo2022attention,
  title={Attention mechanisms in computer vision: A survey},
  author={Guo, Meng-Hao and Xu, Tian-Xing and Liu, Jiang-Jiang and Liu, Zheng-Ning and Jiang, Peng-Tao and Mu, Tai-Jiang and Zhang, Song-Hai and Martin, Ralph R and Cheng, Ming-Ming and Hu, Shi-Min},
  journal={Computational visual media},
  volume={8},
  number={3},
  pages={331--368},
  year={2022},
  publisher={Springer}
}

@article{galvao2023pedestrian,
  title={Pedestrian and vehicle behaviour prediction in autonomous vehicle system—A review},
  author={Galv{\~a}o, Luiz G and Huda, M Nazmul},
  journal={Expert Systems with Applications},
  pages={121983},
  year={2023},
  publisher={Elsevier}
}

@article{mo2023pvdet,
  title={PVDet: Towards pedestrian and vehicle detection on gigapixel-level images},
  author={Mo, Wanghao and Zhang, Wendong and Wei, Hongyang and Cao, Ruyi and Ke, Yan and Luo, Yiwen},
  journal={Engineering Applications of Artificial Intelligence},
  volume={118},
  pages={105705},
  year={2023},
  publisher={Elsevier}
}




@article{kuwornu2016philosophy,
  title={The philosophy behind some Adinkra symbols and their communicative values in Akan},
  author={Kuwornu-Adjaottor, JET and Appiah, George and Nartey, Melvin},
  journal={Philosophical Papers and Review},
  volume={7},
  number={3},
  pages={22--33},
  year={2016},
  publisher={Academic Journals}
}

@inproceedings{chunfa2021perception,
  title={Perception difference analysis using digital technology: case study on Ghanaian Adinkra symbols and Chinese traditional symbols},
  author={Chunfa, Sha and Donkor, Edwin Kofi Nyefrer and Peng, Yao},
  booktitle={E3S Web of Conferences},
  volume={236},
  pages={05016},
  year={2021},
  organization={EDP Sciences}
}

@article{blount2022adinkra,
  title={Adinkra symbolism, printmaking, and the cultural identity of Ghanaian emerging young adults},
  author={Blount, Taheera N and Brookins, Craig C},
  journal={Journal of Creativity in Mental Health},
  volume={17},
  number={3},
  pages={374--393},
  year={2022},
  publisher={Taylor \& Francis}
}

@article{aidoo2022visual,
  title={Visual nexus of Akan adinkra symbols: Some selected works of three contemporary Ghanaian artists},
  author={AIDOO, JOHN BENJAMIN KOFI and AGBESHIE, ABRAHAM},
  journal={Journal of African Art Education. https://www. jaae. atagonline. org},
  volume={2},
  number={1},
  year={2022}
}
Jayasurya, K, et al. "Comparison of Bayesian Network and Support Vector Machine Models for Two-year Survival Prediction in Lung Cancer Patients Treated with Radiotherapy." 2010,  https://doi.org/10.1118/1.3352709.

from the knowledge and expertise of 

Srinivas, S., & Rajendran, S. (2019). Topic-based knowledge mining of online student reviews for strategic planning in universities. Computers & Industrial Engineering. https://doi.org/10.1016/j.cie.2018.06.034

@article{SRINIVAS2019974,
title = {Topic-based knowledge mining of online student reviews for strategic planning in universities},
journal = {Computers & Industrial Engineering},
volume = {128},
pages = {974-984},
year = {2019},
issn = {0360-8352},
doi = {https://doi.org/10.1016/j.cie.2018.06.034},
url = {https://www.sciencedirect.com/science/article/pii/S0360835218303127},
author = {Sharan Srinivas and Suchithra Rajendran}
}

@misc{mitchell1997machine,
  title={Machine learning},
  author={Mitchell, Tom M},
  year={1997}
}

@article{jordan2015machine,
  title={Machine learning: Trends, perspectives, and prospects},
  author={Jordan, Michael I and Mitchell, Tom M},
  journal={Science},
  volume={349},
  number={6245},
  pages={255--260},
  year={2015},
  publisher={American Association for the Advancement of Science}
}

@article{paleyes2022challenges,
  title={Challenges in deploying machine learning: a survey of case studies},
  author={Paleyes, Andrei and Urma, Raoul-Gabriel and Lawrence, Neil D},
  journal={ACM Computing Surveys},
  volume={55},
  number={6},
  pages={1--29},
  year={2022},
  publisher={ACM New York, NY}
}

@article{burkart2021survey,
  title={A survey on the explainability of supervised machine learning},
  author={Burkart, Nadia and Huber, Marco F},
  journal={Journal of Artificial Intelligence Research},
  volume={70},
  pages={245--317},
  year={2021}
}

@book{murphy2022probabilistic,
  title={Probabilistic machine learning: an introduction},
  author={Murphy, Kevin P},
  year={2022},
  publisher={MIT press}
}

@article{nevatia1980linear,
  title={Linear feature extraction and description},
  author={Nevatia, Ramakant and Babu, K Ramesh},
  journal={Computer graphics and image processing},
  volume={13},
  number={3},
  pages={257--269},
  year={1980},
  publisher={Elsevier}
}

@inproceedings{khalid2014survey,
  title={A survey of feature selection and feature extraction techniques in machine learning},
  author={Khalid, Samina and Khalil, Tehmina and Nasreen, Shamila},
  booktitle={2014 science and information conference},
  pages={372--378},
  year={2014},
  organization={IEEE}
}

@book{nixon2019feature,
  title={Feature extraction and image processing for computer vision},
  author={Nixon, Mark and Aguado, Alberto},
  year={2019},
  publisher={Academic press}
}


@article{debnath2021analysis,
  title={Analysis of earthquake forecasting in India using supervised machine learning classifiers},
  author={Debnath, Papiya and Chittora, Pankaj and Chakrabarti, Tulika and Chakrabarti, Prasun and Leonowicz, Zbigniew and Jasinski, Michal and Gono, Radomir and Jasi{\'n}ska, El{\.z}bieta},
  journal={Sustainability},
  volume={13},
  number={2},
  pages={971},
  year={2021},
  publisher={MDPI}
}

@article{bohnslav2021deepethogram,
  title={DeepEthogram, a machine learning pipeline for supervised behavior classification from raw pixels},
  author={Bohnslav, James P and Wimalasena, Nivanthika K and Clausing, Kelsey J and Dai, Yu Y and Yarmolinsky, David A and Cruz, Tom{\'a}s and Kashlan, Adam D and Chiappe, M Eugenia and Orefice, Lauren L and Woolf, Clifford J and others},
  journal={Elife},
  volume={10},
  pages={e63377},
  year={2021},
  publisher={eLife Sciences Publications Limited}
}


@inproceedings{amruthnath2018research,
  title={A research study on unsupervised machine learning algorithms for early fault detection in predictive maintenance},
  author={Amruthnath, Nagdev and Gupta, Tarun},
  booktitle={2018 5th international conference on industrial engineering and applications (ICIEA)},
  pages={355--361},
  year={2018},
  organization={IEEE}
} 

@article{alloghani2020systematic,
  title={A systematic review on supervised and unsupervised machine learning algorithms for data science},
  author={Alloghani, Mohamed and Al-Jumeily, Dhiya and Mustafina, Jamila and Hussain, Abir and Aljaaf, Ahmed J},
  journal={Supervised and unsupervised learning for data science},
  pages={3--21},
  year={2020},
  publisher={Springer}
}


@article{lee2023lftk,
  title={LFTK: Handcrafted Features in Computational Linguistics},
  author={Lee, Bruce W and Lee, Jason Hyung-Jong},
  journal={arXiv preprint arXiv:2305.15878},
  year={2023}
}


@article{zhu2005semi,
  title={Semi-supervised learning literature survey},
  author={Zhu, Xiaojin Jerry},
  year={2005},
  publisher={University of Wisconsin-Madison Department of Computer Sciences}
}

@article{zhou2021semi,
  title={Semi-supervised learning},
  author={Zhou, Zhi-Hua and Zhou, Zhi-Hua},
  journal={Machine Learning},
  pages={315--341},
  year={2021},
  publisher={Springer}
}

@book{zhu2022introduction,
  title={Introduction to semi-supervised learning},
  author={Zhu, Xiaojin and Goldberg, Andrew B},
  year={2022},
  publisher={Springer Nature}
}

@inproceedings{zheng2022simmatch,
  title={Simmatch: Semi-supervised learning with similarity matching},
  author={Zheng, Mingkai and You, Shan and Huang, Lang and Wang, Fei and Qian, Chen and Xu, Chang},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={14471--14481},
  year={2022}
}

@article{song2022graph,
  title={Graph-based semi-supervised learning: A comprehensive review},
  author={Song, Zixing and Yang, Xiangli and Xu, Zenglin and King, Irwin},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  year={2022},
  publisher={IEEE}
}

@article{kaelbling1996reinforcement,
  title={Reinforcement learning: A survey},
  author={Kaelbling, Leslie Pack and Littman, Michael L and Moore, Andrew W},
  journal={Journal of artificial intelligence research},
  volume={4},
  pages={237--285},
  year={1996}
}

@article{li2017deep,
  title={Deep reinforcement learning: An overview},
  author={Li, Yuxi},
  journal={arXiv preprint arXiv:1701.07274},
  year={2017}
}

@article{ladosz2022exploration,
  title={Exploration in deep reinforcement learning: A survey},
  author={Ladosz, Pawel and Weng, Lilian and Kim, Minwoo and Oh, Hyondong},
  journal={Information Fusion},
  volume={85},
  pages={1--22},
  year={2022},
  publisher={Elsevier}
}

@article{raji2020novel,
  title={A novel respiration pattern biometric prediction system based on artificial neural network},
  author={Raji, Rafiu King and Adjeisah, Michael and Miao, Xuhong and Wan, Ailan},
  journal={Sensor Review},
  volume={40},
  number={1},
  pages={8--16},
  year={2020},
  publisher={Emerald Publishing Limited}
}

@article{otchere2021application,
  title={Application of supervised machine learning paradigms in the prediction of petroleum reservoir properties: Comparative analysis of ANN and SVM models},
  author={Otchere, Daniel Asante and Ganat, Tarek Omar Arbi and Gholami, Raoof and Ridha, Syahrir},
  journal={Journal of Petroleum Science and Engineering},
  volume={200},
  pages={108182},
  year={2021},
  publisher={Elsevier}
}


@article{lecun2015deep,
  title={Deep learning},
  author={LeCun, Yann and Bengio, Yoshua and Hinton, Geoffrey},
  journal={nature},
  volume={521},
  number={7553},
  pages={436--444},
  year={2015},
  publisher={Nature Publishing Group UK London}
}

@article{guo2016deep,
  title={Deep learning for visual understanding: A review},
  author={Guo, Yanming and Liu, Yu and Oerlemans, Ard and Lao, Songyang and Wu, Song and Lew, Michael S},
  journal={Neurocomputing},
  volume={187},
  pages={27--48},
  year={2016},
  publisher={Elsevier}
}

@article{niu2021review,
  title={A review on the attention mechanism of deep learning},
  author={Niu, Zhaoyang and Zhong, Guoqiang and Yu, Hui},
  journal={Neurocomputing},
  volume={452},
  pages={48--62},
  year={2021},
  publisher={Elsevier}
}

@article{janiesch2021machine,
  title={Machine learning and deep learning},
  author={Janiesch, Christian and Zschech, Patrick and Heinrich, Kai},
  journal={Electronic Markets},
  volume={31},
  number={3},
  pages={685--695},
  year={2021},
  publisher={Springer}
}

@article{hu2021model,
  title={Model complexity of deep learning: A survey},
  author={Hu, Xia and Chu, Lingyang and Pei, Jian and Liu, Weiqing and Bian, Jiang},
  journal={Knowledge and Information Systems},
  volume={63},
  pages={2585--2619},
  year={2021},
  publisher={Springer}
}

@article{alzubaidi2021review,
  title={Review of deep learning: Concepts, CNN architectures, challenges, applications, future directions},
  author={Alzubaidi, Laith and Zhang, Jinglan and Humaidi, Amjad J and Al-Dujaili, Ayad and Duan, Ye and Al-Shamma, Omran and Santamar{\'\i}a, Jos{\'e} and Fadhel, Mohammed A and Al-Amidie, Muthana and Farhan, Laith},
  journal={Journal of big Data},
  volume={8},
  pages={1--74},
  year={2021},
  publisher={Springer}
}

@article{liu2021efficient,
  title={Efficient extraction of deep image features using convolutional neural network (CNN) for applications in detecting and analysing complex food matrices},
  author={Liu, Yao and Pu, Hongbin and Sun, Da-Wen},
  journal={Trends in Food Science \& Technology},
  volume={113},
  pages={193--204},
  year={2021},
  publisher={Elsevier}
}

@inproceedings{qiu2021deepsweep,
  title={Deepsweep: An evaluation framework for mitigating DNN backdoor attacks using data augmentation},
  author={Qiu, Han and Zeng, Yi and Guo, Shangwei and Zhang, Tianwei and Qiu, Meikang and Thuraisingham, Bhavani},
  booktitle={Proceedings of the 2021 ACM Asia Conference on Computer and Communications Security},
  pages={363--377},
  year={2021}
}

@article{zhang2021deep,
  title={Deep reinforcement learning based resource management for DNN inference in industrial IoT},
  author={Zhang, Weiting and Yang, Dong and Peng, Haixia and Wu, Wen and Quan, Wei and Zhang, Hongke and Shen, Xuemin},
  journal={IEEE Transactions on Vehicular Technology},
  volume={70},
  number={8},
  pages={7605--7618},
  year={2021},
  publisher={IEEE}
}

@inproceedings{sutskever2011generating,
  title={Generating text with recurrent neural networks},
  author={Sutskever, Ilya and Martens, James and Hinton, Geoffrey E},
  booktitle={Proceedings of the 28th international conference on machine learning (ICML-11)},
  pages={1017--1024},
  year={2011}
}

@article{lipton2015critical,
  title={A critical review of recurrent neural networks for sequence learning},
  author={Lipton, Zachary C and Berkowitz, John and Elkan, Charles},
  journal={arXiv preprint arXiv:1506.00019},
  year={2015}
}


@article{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}


@inproceedings{wolf2020transformers,
  title={Transformers: State-of-the-art natural language processing},
  author={Wolf, Thomas and Debut, Lysandre and Sanh, Victor and Chaumond, Julien and Delangue, Clement and Moi, Anthony and Cistac, Pierric and Rault, Tim and Louf, R{\'e}mi and Funtowicz, Morgan and others},
  booktitle={Proceedings of the 2020 conference on empirical methods in natural language processing: system demonstrations},
  pages={38--45},
  year={2020}
}

@article{khan2022transformers,
  title={Transformers in vision: A survey},
  author={Khan, Salman and Naseer, Muzammal and Hayat, Munawar and Zamir, Syed Waqas and Khan, Fahad Shahbaz and Shah, Mubarak},
  journal={ACM computing surveys (CSUR)},
  volume={54},
  number={10s},
  pages={1--41},
  year={2022},
  publisher={ACM New York, NY}
}


@article{mason1999boosting,
  title={Boosting algorithms as gradient descent},
  author={Mason, Llew and Baxter, Jonathan and Bartlett, Peter and Frean, Marcus},
  journal={Advances in neural information processing systems},
  volume={12},
  year={1999}
}

@incollection{bottou2012stochastic,
  title={Stochastic gradient descent tricks},
  author={Bottou, L{\'e}on},
  booktitle={Neural Networks: Tricks of the Trade: Second Edition},
  pages={421--436},
  year={2012},
  publisher={Springer}
} 
@article{ruder2016overview,
  title={An overview of gradient descent optimization algorithms},
  author={Ruder, Sebastian},
  journal={arXiv preprint arXiv:1609.04747},
  year={2016}
}

@inproceedings{ciregan2012multi,
  title={Multi-column deep neural networks for image classification},
  author={Ciregan, Dan and Meier, Ueli and Schmidhuber, J{\"u}rgen},
  booktitle={2012 IEEE conference on computer vision and pattern recognition},
  pages={3642--3649},
  year={2012},
  organization={IEEE}
}

@article{chan2015pcanet,
  title={PCANet: A simple deep learning baseline for image classification?},
  author={Chan, Tsung-Han and Jia, Kui and Gao, Shenghua and Lu, Jiwen and Zeng, Zinan and Ma, Yi},
  journal={IEEE transactions on image processing},
  volume={24},
  number={12},
  pages={5017--5032},
  year={2015},
  publisher={IEEE}
}

@inproceedings{li2013adaptive,
  title={Adaptive active learning for image classification},
  author={Li, Xin and Guo, Yuhong},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={859--866},
  year={2013}
}

@article{wang2021comparative,
  title={Comparative analysis of image classification algorithms based on traditional machine learning and deep learning},
  author={Wang, Pin and Fan, En and Wang, Peng},
  journal={Pattern Recognition Letters},
  volume={141},
  pages={61--67},
  year={2021},
  publisher={Elsevier}
}

@article{traore2018deep,
  title={Deep convolution neural network for image recognition},
  author={Traore, Boukaye Boubacar and Kamsu-Foguem, Bernard and Tangara, Fana},
  journal={Ecological informatics},
  volume={48},
  pages={257--268},
  year={2018},
  publisher={Elsevier}
}

@article{weiss2016survey,
  title={A survey of transfer learning},
  author={Weiss, Karl and Khoshgoftaar, Taghi M and Wang, DingDing},
  journal={Journal of Big data},
  volume={3},
  number={1},
  pages={1--40},
  year={2016},
  publisher={SpringerOpen}
}

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@article{simonyan2014very,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1409.1556},
  year={2014}
}

@inproceedings{szegedy2015going,
  title={Going deeper with convolutions},
  author={Szegedy, Christian and Liu, Wei and Jia, Yangqing and Sermanet, Pierre and Reed, Scott and Anguelov, Dragomir and Erhan, Dumitru and Vanhoucke, Vincent and Rabinovich, Andrew},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1--9},
  year={2015}
}

@article{isinkaye2015recommendation,
  title={Recommendation systems: Principles, methods and evaluation},
  author={Isinkaye, Folasade Olubusola and Folajimi, Yetunde O and Ojokoh, Bolande Adefowoke},
  journal={Egyptian informatics journal},
  volume={16},
  number={3},
  pages={261--273},
  year={2015},
  publisher={Elsevier}
}

@inproceedings{chen2021pre,
  title={Pre-trained image processing transformer},
  author={Chen, Hanting and Wang, Yunhe and Guo, Tianyu and Xu, Chang and Deng, Yiping and Liu, Zhenhua and Ma, Siwei and Xu, Chunjing and Xu, Chao and Gao, Wen},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={12299--12310},
  year={2021}
}

@incollection{lecun2002efficient,
  title={Efficient backprop},
  author={LeCun, Yann and Bottou, L{\'e}on and Orr, Genevieve B and M{\"u}ller, Klaus-Robert},
  booktitle={Neural networks: Tricks of the trade},
  pages={9--50},
  year={2002},
  publisher={Springer}
}

@inproceedings{nair2010rectified,
  title={Rectified linear units improve restricted boltzmann machines},
  author={Nair, Vinod and Hinton, Geoffrey E},
  booktitle={Proceedings of the 27th international conference on machine learning (ICML-10)},
  pages={807--814},
  year={2010}
}
